The Hellan-Herrmann-Johnson and TDNNS method for linear and nonlinear shells

In this paper we extend the recently introduced mixed Hellan-Herrmann-Johnson (HHJ) method for nonlinear Koiter shells to nonlinear Naghdi shells by means of a hierarchical approach. The additional shearing degrees of freedom are discretized by H(curl)-conforming N\'ed\'elec finite elements entailing a shear locking free method. By linearizing the models we obtain in the small strain regime linear Kirchhoff-Love and Reissner-Mindlin shell formulations, which reduce for plates to the originally proposed HHJ and TDNNS method for Kirchhoff-Love and Reissner-Mindlin plates, respectively. By using the Regge interpolation operator we obtain locking-free arbitrary order shell methods. Additionally, the methods can be directly applied to structures with kinks and branched shells. Several numerical examples and experiments are performed validating the excellence performance of the proposed shell elements.

==> results_cant_bend.tex <==
\tikzsetnextfilename{result_cant_bend}
\begin{tikzpicture}
	\begin{axis}[
		legend style={at={(1,0)}, anchor=south east},
		xlabel={displacement},
		ylabel={$P/P_{\mathrm{max}}$},
		]
\addlegendentry{exact}
\addplot[color=black, mark=none] coordinates {
(-0.0, 0.0)
(0.19642028299840852, 0.05)
(0.7741285945363323, 0.1)
(1.6992757039903221, 0.15)
(2.9180792563121187, 0.2)
(4.360562731589024, 0.25)
(5.945386170874743, 0.3)
(7.585403873138709, 0.35)
(9.193532148634088, 0.4)
(10.68849114255538, 0.45)
(12.0, 0.5)
(13.0730527015456, 0.55)
(13.870978567577279, 0.6)
(14.377090222156081, 0.65)
(14.594834498196539, 0.7)
(14.546479089470326, 0.75)
(14.270480185921969, 0.8)
(13.817774875766414, 0.85)
(13.247319045051517, 0.9)
(12.621241037736926, 0.95)
(12.0, 1.0)
};
\addplot[color=black, mark=none, forget plot] coordinates {
(0.0, 0.0)
(1.869503367303345, 0.05)
(3.6475067270129244, 0.1)
(5.248481177042515, 0.15)
(6.598401656263324, 0.2)
(7.639437268410975, 0.25)
(8.333461009842745, 0.3)
(8.664132736140317, 0.35)
(8.637419903760488, 0.4)
(8.280541035200713, 0.45)
(7.639437268410976, 0.5)
(6.774988119709672, 0.55)
(5.758279935840327, 0.6)
(4.665302242537091, 0.65)
(3.5714832899326057, 0.7)
(2.546479089470326, 0.75)
(1.6496004140658265, 0.8)
(0.9262025606545619, 0.85)
(0.4052785252236575, 0.9)
(0.09839491406859713, 0.95)
(0.0, 1.0)
};	


\addlegendentry{TDNNS $p1$ u}
\addplot[color=red, mark=o, mark options={scale=1}] coordinates {	
( 0 , 0.0 )
( 0.19623067041098327 , 0.05 )
( 0.7734072410553199 , 0.1 )
( 1.6977863334166718 , 0.15 )
( 2.9157445923758467 , 0.2 )
( 4.357493907307192 , 0.25 )
( 5.941883387120728 , 0.3 )
( 7.581927111272088 , 0.35 )
( 9.190644786716472 , 0.4 )
( 10.68678309285928 , 0.45 )
( 11.999999999970985 , 0.5 )
( 13.075141257830653 , 0.55 )
( 13.875313511906427 , 0.6 )
( 14.383555792662966 , 0.65 )
( 14.603022393672626 , 0.7 )
( 14.555706313828676 , 0.75 )
( 14.279844109257967 , 0.8 )
( 13.82624129290304 , 0.85 )
( 13.253834664119386 , 0.9 )
( 12.624858314277251 , 0.95 )
( 11.999999999808507 , 1.0 )
};

\addlegendentry{TDNNS $p1$ v}
\addplot[color=blue, mark=o, mark options={scale=1}] coordinates {	
	( 0 , 0.0 )
( 1.869533398976229 , 0.05 )
( 3.6477411089469096 , 0.1 )
( 5.249240049224247 , 0.15 )
( 6.600097888862747 , 0.2 )
( 7.6425060926434245 , 0.25 )
( 8.338282178011191 , 0.3 )
( 8.67095626542529 , 0.35 )
( 8.646306289888523 , 0.4 )
( 8.291325236351932 , 0.45 )
( 7.651722928039667 , 0.5 )
( 6.788174745283184 , 0.55 )
( 5.771621522710617 , 0.6 )
( 4.677991639181983 , 0.65 )
( 3.582752961261995 , 0.7 )
( 2.5557063138493614 , 0.75 )
( 1.6564037026130591 , 0.8 )
( 0.9305164156616568 , 0.85 )
( 0.4073955781978966 , 0.9 )
( 0.09896783439125284 , 0.95 )
( 1.6837066794842147e-10 , 1.0 )
};
%
\addlegendentry{TDNNS $p2$ u}
\addplot[color=teal, mark=x, mark options={scale=1}] coordinates {	
	( 0 , 0.0 )
	( 0.1964274780801749 , 0.05 )
	( 0.7741613390711032 , 0.1 )
	( 1.6993632777913636 , 0.15 )
	( 2.9182659809120683 , 0.2 )
	( 4.3609075578871535 , 0.25 )
	( 5.945956449073111 , 0.3 )
	( 7.586262684560418 , 0.35 )
	( 9.19471956734335 , 0.4 )
	( 10.690001080938584 , 0.45 )
	( 12.001755758854834 , 0.5 )
	( 13.074885769525695 , 0.55 )
	( 13.87261628832994 , 0.6 )
	( 14.37815832024992 , 0.65 )
	( 14.594879803440275 , 0.7 )
	( 14.545015905602904 , 0.75 )
	( 14.267060578059528 , 0.8 )
	( 13.812078904684574 , 0.85 )
	( 13.239256120527894 , 0.9 )
	( 12.611048802442786 , 0.95 )
	( 11.988323374932484 , 1.0 )
};

\addlegendentry{TDNNS $p2$ v}
\addplot[color=orange, mark=x, mark options={scale=1}] coordinates {	
	( 0 , 0.0 )
	( 3.6475141033647387 , 0.1 )
	( 5.248501003818754 , 0.15 )
	( 6.598432497022529 , 0.2 )
	( 7.639459183526987 , 0.25 )
	( 8.333423944791736 , 0.3 )
	( 8.663946815411101 , 0.35 )
	( 8.636950641793929 , 0.4 )
	( 8.279612577416557 , 0.45 )
	( 7.637846346230542 , 0.5 )
	( 6.772530302559046 , 0.55 )
	( 5.7547879470879995 , 0.6 )
	( 4.660693675655573 , 0.65 )
	( 3.5658122845410505 , 0.7 )
	( 2.5399838338882668 , 0.75 )
	( 1.642736278298908 , 0.8 )
	( 0.9196498167705508 , 0.85 )
	( 0.3999145007423742 , 0.9 )
	( 0.0952233878746646 , 0.95 )
	( 3.576105746844037e-05 , 1.0 )
	
};

\end{axis}
\end{tikzpicture}


==> results_cant_shear.tex <==
\tikzsetnextfilename{result_cant_shear}
\begin{tikzpicture}
	\begin{axis}[
		legend style={at={(1,0)}, anchor=south east},
		xlabel={displacement},
		ylabel={$P/P_{\mathrm{max}}$},
		]
\addlegendentry{Sze et al. 2004}
\addplot[color=black, mark=none] coordinates {
(-0.0, 0.0)
(0.663,0.05)
(1.309,0.1)
(1.922,0.15)
(2.493,0.2)
(3.015,0.25)
(3.488,0.3)
(3.912,0.35)
(4.292,0.4)
(4.631,0.45)
(4.933,0.5)
(5.202,0.55)
(5.444,0.6)
(5.660,0.65)
(5.855,0.7)
(6.031,0.75)
(6.190,0.8)
(6.335,0.85)
(6.467,0.9)
(6.588,0.95)
(6.698,1)
};
\addplot[color=black, mark=none, forget plot] coordinates {
(0.0, 0.0)
(0.026,0.05)
(0.103,0.1)
(0.224,0.15)
(0.381,0.2)
(0.563,0.25)
(0.763,0.3)
(0.971,0.35)
(1.184,0.4)
(1.396,0.45)
(1.604,0.5)
(1.807,0.55)
(2.002,0.6)
(2.190,0.65)
(2.370,0.7)
(2.541,0.75)
(2.705,0.8)
(2.861,0.85)
(3.010,0.9)
(3.151,0.95)
(3.286,1)
};	


\addlegendentry{TDNNS $p1$ u}
\addplot[color=red, mark=o, mark options={scale=1}] coordinates {	
( 0 , 0.0 )
( 0.6645631440980972 , 0.05 )
( 1.3115539857255076 , 0.1 )
( 1.9261253191520384 , 0.15 )
( 2.4978814350408456 , 0.2 )
( 3.021236147154186 , 0.25 )
( 3.4947150556123407 , 0.3 )
( 3.919789856722904 , 0.35 )
( 4.299721314778022 , 0.4 )
( 4.638646550791406 , 0.45 )
( 4.940958092220684 , 0.5 )
( 5.210929362496369 , 0.55 )
( 5.452516454771678 , 0.6 )
( 5.669273260882112 , 0.65 )
( 5.864333546700145 , 0.7 )
( 6.040429224304619 , 0.75 )
( 6.199925858019808 , 0.8 )
( 6.3448643909777305 , 0.85 )
( 6.4770030773508624 , 0.9 )
( 6.5978566091287005 , 0.95 )
( 6.708731153211584 , 1.0 )
};

\addlegendentry{TDNNS $p1$ v}
\addplot[color=blue, mark=x, mark options={scale=1}] coordinates {	
( 0 , 0.0 )
( 0.026503915268566887 , 0.05 )
( 0.10368746522529232 , 0.1 )
( 0.2251917393975085 , 0.15 )
( 0.382176456504272 , 0.2 )
( 0.5650785060890877 , 0.25 )
( 0.7649814364713671 , 0.3 )
( 0.9743746349595824 , 0.35 )
( 1.1873859294669389 , 0.4 )
( 1.3996855354832876 , 0.45 )
( 1.6082402944841183 , 0.5 )
( 1.8110337214297585 , 0.55 )
( 2.0068101250759574 , 0.6 )
( 2.19486415242738 , 0.65 )
( 2.3748778298546678 , 0.7 )
( 2.5467990520839363 , 0.75 )
( 2.7107532232296645 , 0.8 )
( 2.866980151501408 , 0.85 )
( 3.0157896144137646 , 0.9 )
( 3.1575304691937034 , 0.95 )
( 3.292569466568912 , 1.0 )	
};

\end{axis}
\end{tikzpicture}

